Abstract interpretation-based approaches to Security - A Survey on Abstract Non-Interference and its Challenging Applications

In this paper we provide a survey on the framework of abstract non-interference. In particular, we describe a general formalization of abstract non-interference by means of three dimensions (observation, protection and semantics) that can be instantiated in order to obtain well known or even new weakened non-interference properties. Then, we show that the notions of abstract non-interference introduced in language-based security are instances of this more general framework which allows to better understand the different components of a non-interference policy. Finally, we consider two challenging research fields concerning security where abstract non-interference seems a promising approach providing new perspectives and new solutions to open problems: Code injection and code obfuscation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{41}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.4}{10.4204/EPTCS.129.4}}
\pdfoutput=1

